Semantic Similarity-Based Clustering of Findings From Security Testing Tools

Over the last years, software development in domains with high security demands transitioned from traditional methodologies to uniting modern approaches from software development and operations (DevOps). Key principles of DevOps gained more importance and are now applied to security aspects of software development, resulting in the automation of security-enhancing activities. In particular, it is common practice to use automated security testing tools that generate reports after inspecting a software artifact from multiple perspectives. However, this raises the challenge of generating duplicate security findings. To identify these duplicate findings manually, a security expert has to invest resources like time, effort, and knowledge. A partial automation of this process could reduce the analysis effort, encourage DevOps principles, and diminish the chance of human error. In this study, we investigated the potential of applying Natural Language Processing for clustering semantically similar security findings to support the identification of problem-specific duplicate findings. Towards this goal, we developed a web application for annotating and assessing security testing tool reports and published a human-annotated corpus of clustered security findings. In addition, we performed a comparison of different semantic similarity techniques for automatically grouping security findings. Finally, we assess the resulting clusters using both quantitative and qualitative evaluation methods.

==> section/abstract.tex <==
\begin{abstract}
%Fast pace in DevOps and relevancy of cybersecurity
Over the last decade, software development in domains with high security demand like industrial systems, transitioned from traditional methodologies to modern DevOps approaches. 
%Automated code analysis with security testing tools, resulting into duplicates
Key principles of DevOps are applied to all aspects of software development including security, resulting in automation of security activities. In particular the automation of security tests generates reports frequently, which inspect the software from multiple perspectives. This introduces the challenge of duplicate security findings. 
%Problem: time cost, repetitive, manual checks can lead to human error, hinderance of agility
To repeatedly identify these duplicates manually, a domain expert has to invest time, effort and knowledge. An automated approach supporting this process could reduce analysis effort, encourage DevOps principles and diminish human error.  

%RQ: How do semantic similarity techniques from NLP perform in the task semantically grouping security tool reports?
In this paper, we investigate the potential of Natural Language Processing for the identification of duplicate security findings in DevOps projects. 
%Contributions are two-fold (1) annotation tool and human-annotated corpus of deduplicated security tool reports (2) comparison different semantic similarity techniques for clustering security findings + insights from evaluation for scholars and practitioners
Towards this goal we contribute a tool for the annotation and evaluation of security findings by security professionals, complemented with a human-annotated corpus of deduplicated security tool findings. Second, we provide a comparison of different semantic similarity techniques for the clustering of security findings, further refined by the insights from an industrial practitioner. 
\textcolor{red}{20/08/22 Phillip: created outline of paper, let's discuss on Monday}
\textcolor{red}{24/08/22 Markus: First Draft}
\end{abstract}
